Restoring AC Power Flow Feasibility from Relaxed and Approximated Optimal Power Flow Models

To address computational challenges associated with power flow nonconvexities, significant research efforts over the last decade have developed convex relaxations and approximations of optimal power flow (OPF) problems. However, benefits associated with the convexity of these relaxations and approximations can have tradeoffs in terms of solution accuracy since they may yield voltage phasors that are inconsistent with the power injections and line flows, limiting their usefulness for some applications. Inspired by state estimation (SE) techniques, this paper proposes a new method for obtaining an AC power flow feasible point from the solution to a relaxed or approximated optimal power flow (OPF) problem. By treating the inconsistent voltage phasors, power injections, and line flows analogously to noisy measurements in a state estimation algorithm, the proposed method yields power injections and voltage phasors that are feasible with respect to the AC power flow equations while incorporating information from many quantities in the solution to a relaxed or approximated OPF problem. We improve this method by adjusting weighting terms with an approach inspired by algorithms used to train machine learning models. We demonstrate the proposed method using several relaxations and approximations. The results show up to several orders of magnitude improvement in accuracy over traditional methods.

==> Comments/Comments.tex <==
Review of Restoring AC Power Flow Feasibility from Relaxed and Approximated Optimal
Power Flow Models
The present paper proposes a machine learning-based approach to restore the feasible
solution of non-convex AC-OPF. The overall presentation is ok, yet can be improved. The
details are as follows.


1. Except for the gradient descent part (AdaGrad part), I cannot find how the machine
learning approach gets involved. It seems this paper does not use any classical or
deep learning approaches.

2. The preliminaries part may be a little bit redundant. SDP, SOCP, and QC are all
pretty common and it seems this paper does not have any modifications or
improvements on these methods.

3. The paper states that Eq.10 leverages more information than existing restoration
methods. Could you please elaborate more on this?

4. Eq.12 has a similar format as the L2 loss. Maybe cannot be treated as a main
contribution of the paper.

5. It is probably better to compare with some existing restoration methods in numerical
results. This paper seems not to compare with any competitors.

6. Table II shows the mean square loss, and sometimes the benchmark performs
better. It is better to highlight the winners for the readers.

7. This algorithm relies on solvers to solve AC-OPF, which can be pretty
time-consuming. The computational time of data generation progress may be much
longer than solving the original AC-PF problems using the NR method. Probably this
paper should address the selling points.










The goal of is paper is to find feasible solutions to AC
optimal power flow equations from the solution to a relaxed
or approximated optimal power flow (OPF) problem. It is
pretty important in both research and reality. The idea of
this paper is interesting but straightforward. It treats
the obtained solutions to a relaxed or approximated optimal
power flow (OPF) problem analogously to noisy measurements
in a state estimation algorithm. Then, it calculates the
feasible solution through weighted least square
formulation, where a machine learning approach can obtain
the weight parameters.
Overall, the description of the proposed approach is easy
to follow. However, in this paper, the authors did not
discuss the recent approach directly applying machine
learning to solve the OPF problem, like the followings:

[1] X. Pan, T. Zhao, M. Chen and S. Zhang, "DeepOPF: A Deep
Neural Network Approach for Security-Constrained DC Optimal
Power Flow", in IEEE Transactions on Power Systems, vol.
36, no. 3, pp. 1725 - 1735, May. 2021.
[2] X. Pan, M. Chen, T. Zhao and S. H. Low, "DeepOPF: A
Feasibility-Optimized Deep Neural Network Approach for AC
Optimal Power Flow Problems", arXiv preprint
arXiv:2007.01002, 2020.
[3] A. Zamzam and K. Baker, "Learning Optimal Solutions for
Extremely Fast AC Optimal Power Flow", in Proceedings of
the 11th IEEE International Conference on Communications,
Control, and Computing Technologies for Smart Grids (IEEE
SmartGridComm 2020), virtual conference, Nov. 11 - 13,
2020.
Indeed, this approach is related to the topic of this
paper. The authors had better add related papers for
discussion.












In this paper, the authors present a method to take a solution of a relaxed
OPF problem, and generate a `consistent' solution which is feasible for AC-OPF.
The inconsistencies between AC-feasible and AC-infeasible solutions are mod-
eled as sensor errors, and state estimation techniques are brought in. In order
to estimate the variance of each of the `sensors', a machine learning technique is
used, which creates a dataset of the form fxAC; xR( )g, and the sensor variance
  is chosen as the one which can best explain the discrepancy in this dataset.
The reviewer feels that the paper is well written and justi ed through sim-
ulations, yet certain approaches presented in the paper may be too ad-hoc.
Speci c comments follow.
• How does the current method compare to other approaches for AC feasi-
bility restoration in literature, for example [1]?
• Since it is stated that AC-OPF solutions are hard to  nd due to non-
convexity, how do the authors generate xAC in Section III.B?
• How do the authors ensure that the data points xAC will be represen-
tative for all scenarios during testing phase? In case the dataset is not
representative of the testing phase, how will the wrong value of   a ect
performance?
• Shouldn't the term vec(@xR)
vec(@ ) actually be @vec(xR)
@vec( ) ?
References
[1] X. Fang, Z. Yang, J. Yu, and Y. Wang, \Ac feasibility restoration in market
clearing: Problem formulation and improvement," IEEE Transactions on
Industrial Informatics, vol. 18, no. 11, pp. 7597{7607, 2022.
